One-loop calculations in quantum field theory: from Feynman diagrams to unitarity cuts

The success of the experimental program at the Tevatron re-inforced the idea that precision physics at hadron colliders is desirable and, indeed, possible. The Tevatron data strongly suggests that one-loop computations in QCD describe hard scattering well. Extrapolating this observation to the LHC, we conclude that knowledge of many short-distance processes at next-to-leading order may be required to describe the physics of hard scattering. While the field of one-loop computations is quite mature, parton multiplicities in hard LHC events are so high that traditional computational techniques become inefficient. Recently new approaches based on unitarity have been developed for calculating one-loop scattering amplitudes in quantum field theory. These methods are especially suitable for the description of multi-particle processes in QCD and are amenable to numerical implementations. We present a systematic pedagogical description of both conceptual and technical aspects of the new methods.

==> mainfiles.tex <==
\input{B1/Section1.tex} 
\input{B2/Section2.tex}
\input{B3/Section3.tex}
\input{B4/Section4.tex}
\input{B5/Section5.tex}
\input{B6/Section6.tex}
\input{B7/Section7.tex}
\input{B8/Section8.tex}
\input{B9/Section9.tex}
\input{B10/Section10.tex}
\input{B11/Section11.tex}
\input{App1/Appendix1.tex}
\input{App2/Appendix2.tex}
\input{App3/Appendix3.tex}
\input{App4/Appendix4.tex}
\input{App5/Appendix5.tex}
\addcontentsline{toc}{section}{Bibliography}


==> newcomamm.tex <==
\def\e{\epsilon}
\def\sud{s_{12}}
\def\sdt{s_{23}}
\def\phase{e^{- i \lambda_{ij} \pi}}
\def\zb{\bar{z}}
\def\abs#1{|#1|}
\def\spab#1.#2.#3{\langle\mskip-1mu{#1} 
                  | #2 | {#3}\mskip-1mu]}
\def\spba#1.#2.#3{[\mskip-1mu{#1} 
                  | #2 | {#3}\mskip-1mu\rangle}
\def\spa#1.#2{\langle#1\,#2\rangle}
\def\spb#1.#2{[#1\,#2]}
\def\cm{{\cal M}}
\def\ep{\epsilon}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\la{\langle}
\def\ra{\rangle}
\def\cg{c_\Gamma}
\def\bom#1{{\mbox{\boldmath $#1$}}}
\def\as{\alpha_S}
\def\Eq{Eq.~}
\def\Eqs{Eqs.~}
\def\tb{\tilde b}
\def\bb{\bar b}
\def\slsh{\rlap{$\;\!\!\not$}}     % Feynman slash
%\def\vNV{vN-V}
\def\vNV{van Neerven - Vermaseren}
\def\Nc{N_c}
%\newcommand{\s}{\slash\hspace{-5pt}}
\newcommand{\ttbs}{\char'134}%\backslash for \tt
\newcommand\fverb{\setbox\fverbbox=\hbox\bgroup\verb}
\newcommand\fverbdo{\egroup\medskip\noindent%
			\fbox{\unhbox\fverbbox}\ }
\newcommand\fverbit{\egroup\item[\fbox{\unhbox\fverbbox}]}
\newbox\fverbbox
\newcommand{\jhepname}{JHEP}
%\newcommand{\gtrsim}{\raisebox{.2em}{$\rlap{\raisebox{-.5em}{$\;\sim$}}>\,$}}
\def\ib{\bar{\imath}}
\def\jb{\bar{\jmath}}
\def\qb{{\bar q}}
\def\Qb{{\bar Q}}
\newcommand{\lb}{{\bar l}}
\newcommand{\qqgggW}{\qb q ggg W}
\newcommand{\qqQQgW}{\qb q \Qb Q g W}
\newcommand{\eps}{\epsilon}
%\newcommand{\e}{\epsilon}
\newcommand{\nn}{\nonumber \\}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\ve}{\varepsilon}

\def\mo{m_1}
\def\mt{m_2}
\def\nh{\hat{n}}
\def\ne{n_{\epsilon}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray}}
\def\lt{l_{(2)}}
\def\nn{\nonumber}


\newbox\charbox
\newbox\slabox

\def\s#1{{      % Feynman slash
        \setbox\charbox=\hbox{$#1$}
        \setbox\slabox=\hbox{$/$}
        \dimen\charbox=\ht\slabox
        \advance\dimen\charbox by -\dp\slabox
        \advance\dimen\charbox by -\ht\charbox
        \advance\dimen\charbox by \dp\charbox
        \divide\dimen\charbox by 2
        \raise-\dimen\charbox\hbox to \wd\charbox{\hss/\hss}
        \llap{$#1$} }}
\def\ksl{\s{k}}

\def\tree{{\rm tree}}
\def\oneloop{{1 \mbox{-} \rm loop}}

\def\nf{n_{\! f}}
\def\Ord{{\cal O}}
\def\A{{\cal A}}
\def\B{{\cal B}}
\def\la{\langle}
\def\ra{\rangle}
\def\sumint#1{\sum \!\!\!\!\!\!\!\! \int_{\raisebox{-.8ex}{#1}}}
\def\ketsub#1{_{\raisebox{-.8ex}{\scriptsize {#1}}}}
\def\ltxt#1#2#3#4{\hspace{#1}\raisebox{#3}{#4}\hspace{#2}}

\def\si{\sigma}


\def\ket#1{|#1]}
\def\aket#1{|#1\rangle}
\newcommand{\bra}[1]{\langle{#1}|}
% define cut properties
\newcommand{\cut}[2]{ \!{\vphantom{\Big|}}_{#1}{\Big|}_{#2}\! }


\newcommand{\epem}{e^+ e^- }
%\newcommand{\half}{\frac{1}{2}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cW}{{\cal W}}
% Journals
\newcommand{\APNY}[1]{{Ann. Phys. N. Y. \textbf{#1}}}
\newcommand{\epj}[1]{{Eur.\ Phys.\ J.\ C \textbf{#1}}}
\newcommand{\EPJ}[1]{{Eur.\ Phys.\ J.\ C \textbf{#1}}}
\newcommand{\JHEP}{J.\ High Energy Phys.\ }
\newcommand{\IJMP}[1]{{Int. J. Mod. Phys. A \textbf{#1}}}
\newcommand{\JL}[1]{{JETP  Lett. \textbf{#1}}}
\newcommand{\lnc}[1]{{Lett. Nuovo Cim. \textbf{#1}}}
\newcommand{\NC}[1]{{Nuovo Cimento \textbf{#1}}}
\newcommand{\NCA}[1]{{Nuovo Cimento A \textbf{#1}}}
\newcommand{\NIM}[1]{{Nucl. Instrum. Methods \textbf{#1}}}
\newcommand{\NIMA}[1]{{Nucl. Instrum. Methods A \textbf{#1}}}
\newcommand{\np}[1]{{Nucl. Phys. B \textbf{#1}}}
\newcommand{\npb}[1]{{Nucl. Phys. B \textbf{#1}}}
\newcommand{\NPB}[1]{{Nucl. Phys. B \textbf{#1}}}
\newcommand{\NPBPS}[1]{{Nucl. Phys. B (Proc. Suppl.) \textbf{#1}}}
\newcommand{\pl}[1]{{Phys. Lett. \textbf{#1}B}}        % Vol 1 to 170
\newcommand{\PLB}[1]{{Phys. Lett. B \textbf{#1}}}
\newcommand{\plb}[1]{{Phys. Lett. B \textbf{#1}}}       % Vol 171 ...
\newcommand{\PR}[1]{{Phys. Rep. C \textbf{#1}}}
\newcommand{\pr}[1]{{Phys. Rev. \textbf{#1}}}
\newcommand{\prd}[1]{{Phys. Rev. D \textbf{#1}}}
\newcommand{\PRD}[1]{{Phys. Rev. D \textbf{#1}}}
\newcommand{\prl}[1]{{Phys. Rev. Lett. \textbf{#1}}}
\newcommand{\PRL}[1]{{Phys. Rev. Lett. \textbf{#1}}}
\newcommand{\ptp}[1]{{Prog. Theor. Phys. \textbf{#1}}}
\newcommand{\SJ}[1]{{Sov. J. Nucl. Phys. \textbf{#1}}}
\newcommand{\SJNP}[1]{{Sov. J. Nucl. Phys. \textbf{#1}}}
\newcommand{\zp}[1]{{Z. Phys. C \textbf{#1}}}
\newcommand{\ZPC}[1]{{Z. Phys. C \textbf{#1}}}
\newcommand{\footnoteremember}[2]{
  \footnote{#2}
  \newcounter{#1}
  \setcounter{#1}{\value{footnote}}
} 
\newcommand{\footnoterecall}[1]{
  \footnotemark[\value{#1}]
} 

